A Strong-QCD Regime Measurement of the Proton's Spin Structure

The theory of the strong force, Quantum Chromodynamics (QCD) remains one of the most important ways to understand the fundamental properties of ordinary matter. However, at low momentum transfer Q2, in the regime where the strong force becomes extremely strong, our understanding of QCD for ordinary nucleons becomes hazy. Several cutting edge theories such as Chiral Perturbation Theory and Lattice QCD have provided valuable predictions in this regime, but Lattice QCD has not yet extended predictions of many important quantities to this kinematic region, and Chiral Perturbation Theory has faced several important disagreements with experimental data for the neutron over the last several decades. It is therefore of extreme importance to have a benchmark of experimental data in the low energy regime for the proton's behavior, as a test of leading theories for the behavior of QCD in this regime. The E08-027 (g2p) experiment ran at Jefferson Lab in 2012 with the goal of collecting this valuable data. Full details of the g2p experiment and my experimental work at the University of New Hampshire are presented in this thesis, as well as a detailed description of the analysis process and the exciting benchmark results, which serve as a direct test of all current and future theories of QCD in the low-Q2 regime.

==> appendices/thingstoadd.tex <==
\chapter{THINGS TO ADD}

Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more. Here I want to write even more.

==> chapters/basics.tex <==
\chapter{BASIC THINGS TO KNOW}




\section{Literature citations}

My books and papers\footnote{Here I'm adding a footnote.} are stored in .bib file and I can refer to them as \cite{popper2002logic} and \cite{schwartz2008importance}.




\section{Writing math}

I can write in-line math like $\alpha^n+\beta^n=\gamma^n$. I also can write displayed math with numbering:
%
\begin{equation}
\label{eqn:mymath}
\int_0^\infty f(x) \, dx = 0
\end{equation}
%
or without:
\[
\sum_{i=0}^\infty f(x_i) \Delta x_i \approx 0.
\]
%
I can refer to the formula \eqref{eqn:mymath} here.





\section{Inserting picture}

I'm inserting and then referring to the Figure \ref{fig:sine}.

\begin{figure}[htb]
\centering
\includegraphics[width=0.7\textwidth]{figures/sine.png}
\caption{Sine function}
\label{fig:sine}
\end{figure}






\section{Inserting table}

I'm inserting and then referring to the Table \ref{tab:constants}.

\begin{table}[htb]
\centering
\begin{tabular}{|c|c|}
\hline
Constant & Value\\
\hline
$\alpha$ & $1$\\
\hline
$\beta$ & $2$\\
\hline
$\gamma$ & $3$\\
\hline
\end{tabular}
\caption{Values of some constants}
\label{tab:constants}
\end{table}






\section{Inserting code}

I want to insert some Python code here:

\singlespacing
\begin{lstlisting}[language=Python]
def greet(name):
    print('Hello', name)
greet('Alice')
greet('Bob')
\end{lstlisting}
\doublespacing





\section{Enumerating}

Here I want to enumerate couple things:

\begin{enumerate}
\item
First thing.
\item
Second thing.
\end{enumerate}





\section{In case I have questions about \LaTeX}

\url{google.com}


==> frontmatter/listofsymbols.tex <==
\chapter*{LIST OF SYMBOLS}
\addcontentsline{toc}{chapter}{LIST OF SYMBOLS}

\noindent $\alpha$ --- some constant ($\si{\N}$)

\noindent $\beta$ --- another constant ($\si{\Hz}$)

\noindent $\gamma$ --- one more constant ($\si{\Pa}$)

\pagebreak

==> frontmatter/preface.tex <==
\chapter*{PREFACE}
\addcontentsline{toc}{chapter}{PREFACE}

Here I'm going to say something to introduce the topic. Here I'm going to say something to introduce the topic. Here I'm going to say something to introduce the topic. Here I'm going to say something to introduce the topic. Here I'm going to say something to introduce the topic. Here I'm going to say something to introduce the topic. Here I'm going to say something to introduce the topic. Here I'm going to say something to introduce the topic.

\pagebreak
